Multi-Dialect Arabic BERT for Country-Level Dialect Identification

Arabic dialect identification is a complex problem for a number of inherent properties of the language itself. In this paper, we present the experiments conducted, and the models developed by our competing team, Mawdoo3 AI, along the way to achieving our winning solution to subtask 1 of the Nuanced Arabic Dialect Identification (NADI) shared task. The dialect identification subtask provides 21,000 country-level labeled tweets covering all 21 Arab countries. An unlabeled corpus of 10M tweets from the same domain is also presented by the competition organizers for optional use. Our winning solution itself came in the form of an ensemble of different training iterations of our pre-trained BERT model, which achieved a micro-averaged F1-score of 26.78% on the subtask at hand. We publicly release the pre-trained language model component of our winning solution under the name of Multi-dialect-Arabic-BERT model, for any interested researcher out there.

==> sections/models/electra.tex <==
\\ELECTRA stands for Efficiently Learning an Encoder that Classifies Token Replacements Accurately \cite{clark2020electra}. This model uses a generator-discriminator model, with the discriminator being the locus of pre-training. The generator is usually a relatively weak BERT-like model (i.e. transformer encoder), which attempts to replace a few tokens in a sentence with others that are somewhat close to the original context. The discriminator, also a BERT-like model, is then tasked with finding which tokens were replaced. 

==> sections/models/ngram_char.tex <==
%\\In this model, we utilize a modified version of CharCNN \cite{zhang2015character} in a distant supervision settings. To build a large enough training set for the CharCNN model, we first train a K-nearest-neighbours classifier on the TF-IDF vectorization of the 21K labeled data and then we weakly classify each of 10M unlabelled data using that classifier. The weakly-labelled 10M tweets is then combined with 21K labelled tweets to form one training set for the CharCNN model. our CharCNN model is the same as the one proposed in \cite{zhang2015character} except that we use five CNNs in the first layer with kernel sizes from 1 to 5 in order to learn character n-gram features. The output of these five CNNs is concatenated into one single vector and passed through the rest of the CharCNN network.
\\In this model, we utilize a modified version of CharCNN \cite{zhang2015character} in a distant supervision settings. To build a large enough training set for the CharCNN model, we first train a K-nearest-neighbours classifier on the TF-IDF vectorization of the 21K labeled data and then we weakly classify each of 10M unlabelled data using that classifier. The weakly-labelled 10M tweets is then combined with 21K labelled tweets to form one training set for the CharCNN model. The output of the CNNs layers is concatenated into one single vector and passed through the rest of the CharCNN network.
